Neural-PIM: Efficient Processing-In-Memory with Neural Approximation of Peripherals

Processing-in-memory (PIM) architectures have demonstrated great potential in accelerating numerous deep learning tasks. Particularly, resistive random-access memory (RRAM) devices provide a promising hardware substrate to build PIM accelerators due to their abilities to realize efficient in-situ vector-matrix multiplications (VMMs). However, existing PIM accelerators suffer from frequent and energy-intensive analog-to-digital (A/D) conversions, severely limiting their performance. This paper presents a new PIM architecture to efficiently accelerate deep learning tasks by minimizing the required A/D conversions with analog accumulation and neural approximated peripheral circuits. We first characterize the different dataflows employed by existing PIM accelerators, based on which a new dataflow is proposed to remarkably reduce the required A/D conversions for VMMs by extending shift and add (S+A) operations into the analog domain before the final quantizations. We then leverage a neural approximation method to design both analog accumulation circuits (S+A) and quantization circuits (ADCs) with RRAM crossbar arrays in a highly-efficient manner. Finally, we apply them to build an RRAM-based PIM accelerator (i.e., \textbf{Neural-PIM}) upon the proposed analog dataflow and evaluate its system-level performance. Evaluations on different benchmarks demonstrate that Neural-PIM can improve energy efficiency by 5.36x (1.73x) and speed up throughput by 3.43x (1.59x) without losing accuracy, compared to the state-of-the-art RRAM-based PIM accelerators, i.e., ISAAC (CASCADE).

==> bib_bak.tex <==

% \bibliographystyle{./IEEEtran}
% \bibliography{./IEEEabrv,./IEEEexample}
% \begin{thebibliography}{99}



%\footnotesize







@inproceedings{googlenet,
  author = {{Szegedy}, C. and {Wei Liu} and {Yangqing Jia} and {Sermanet}, P. and {Reed}, S. and {Anguelov}, D. and {Erhan}, D. and {Vanhoucke}, V. and {Rabinovich}, A.},
  booktitle = {2015 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages = {1-9},
  title = {{Going Deeper with Convolutions}},
  year = 2015,
}



@inproceedings{isaac,
  title={{ISAAC: A Convolutional Neural Network Accelerator with In-situ Analog Arithmetic in Crossbars}},
  author={Shafiee, Ali and et al},
  booktitle={2016 ACM/IEEE 43rd Annual International Symposium on Computer Architecture (ISCA)},
  pages={14--26},
  year={2016},
}


@inproceedings{cascade,
author = {Chou, Teyuh and Tang, Wei and Botimer, Jacob and Zhang, Zhengya},
title = {{CASCADE: Connecting RRAMs to Extend Analog Dataflow In An End-To-End In-Memory Processing Paradigm}},
year = {2019},
booktitle = {Proceedings of the 52nd Annual IEEE/ACM International Symposium on Microarchitecture (MICRO)},
pages = {114--125},
}






@inproceedings{relu,
  title={{Rectified Linear Units Improve Restricted Boltzmann Machines}},
  author={Nair, Vinod and Hinton, Geoffrey E},
  booktitle={Proceedings of the 27th international conference on machine learning (ICML)},
  pages={807--814},
  year={2010}
}



@inproceedings{karpathy2015deep,
  title={{Deep visual-semantic alignments for generating image descriptions}},
  author={Karpathy, Andrej and Fei-Fei, Li},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition (CVPR)},
  pages={3128--3137},
  year={2015}
}







@inproceedings{alexnet,
author = {Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E.},
title = {{ImageNet Classification with Deep Convolutional Neural Networks}},
year = {2012},
booktitle = {Proceedings of the 25th International Conference on Neural Information Processing Systems (NeurIPS)},
pages = {1097–1105},
}



@conference{overfeat,
title = {{Overfeat: Integrated Recognition, Localization and Detection Using Convolutional Networks}},
author = {Pierre Sermanet and David Eigen and Xiang Zhang and Michael Mathieu and Rob Fergus and Yann LeCun},
year = {2014},
pages={1--9},
booktitle = {International Conference on Learning Representations (ICLR)},
}


@INPROCEEDINGS{NLP, 
author={G. {Chen} and et al}, 
booktitle={IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, 
title={{Small-Footprint Keyword Spotting Using Deep Neural Networks}}, 
year={2014},
pages={4087-4091},
}





@article{lecun2015deep,
  title={Deep learning},
  author={LeCun and et al},
  journal={Nature},
  volume={521},
  number={7553},
  pages={436},
  year={2015},
  publisher={Nature Publishing Group}
}

@article{ambrogio2018,
  title={Equivalent-accuracy accelerated neural-network training using analogue memory},
  author={Ambrogio, Stefano and et al},
  journal={Nature},
  volume={558},
  number={7708},
  pages={60},
  year={2018},
  publisher={Nature Publishing Group}
}

@inproceedings{resnet,
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={2016 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={{Deep Residual Learning for Image Recognition}},  year = {2016},
  pages={770--778},
}

@inproceedings{vgg16,
    title={{Very Deep Convolutional Networks for Large-Scale Image Recognition}},
    author={Karen Simonyan and Andrew Zisserman},
    year={2014},
    pages={1--8},
    booktitle = {International Conference on Learning Representations (ICLR)},
}


@INPROCEEDINGS{mobilenetv2,
  author={Sandler, Mark and Howard, Andrew and Zhu, Menglong and Zhmoginov, Andrey and Chen, Liang-Chieh},
  booktitle={2018 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={{MobileNetV2: Inverted Residuals and Linear Bottlenecks}}, 
  year={2018},
  pages={4510-4520},}



@inproceedings{an_1,
author = {Zou, An and Garimella, Karthik and Lee, Benjamin and Gill, Christopher and Zhang, Xuan},
title = {{F-LEMMA: Fast Learning-Based Energy Management for Multi-/Many-Core Processors}},
year = {2020},
booktitle = {Proceedings of the 2020 ACM/IEEE Workshop on Machine Learning for CAD},
pages = {43--48},
}

@INPROCEEDINGS{an_2,
  author={Sun, Jinghao and Li, Jing and Guo, Zhishan and Zou, An and Zhang, Xuan and Agrawal, Kunal and Baruah, Sanjoy},
  booktitle={2020 IEEE Real-Time and Embedded Technology and Applications Symposium (RTAS)}, 
  title={{Real-Time Scheduling upon a Host-Centric Acceleration Architecture with Data Offloading}}, 
  year={2020},
  pages={56-69},}

@inproceedings{zhu2018cmos,
  title={{CMOS Image Sensor Data-Readout Method for Convolutional Operations with Processing Near Sensor Architecture}},
  author={Zhu, Huifeng and et al},
  booktitle={2018 IEEE Asia Pacific Conference on Circuits and Systems (APCCAS)},
  pages={528--531},
  year={2018},
}




@ARTICLE{chen_1,
  author={Zhao, Chenfeng and Zhang, Xuan and Chamberlain, Roger D.},
  journal={IEEE Design \& Test}, 
  title={{Executing Data Integration Effectively and Efficiently Near the Memory}}, 
  year={2021},
  pages={1-1},}
  
  
  

@ARTICLE{feng_1,
  author={Chen, Zhe and et al},
  journal={IEEE Transactions on Circuits and Systems I: Regular Papers (TCAS-I)}, 
  title={{Processing Near Sensor Architecture in Mixed-Signal Domain With CMOS Image Sensor of Convolutional-Kernel-Readout Method}}, 
  year={2020},
  volume={67},
  number={2},
  pages={389-400},}


@incollection{NIPS2019_fix,
title = {Fixing the train-test resolution discrepancy},
author = {Touvron, Hugo and Vedaldi, Andrea and Douze, Matthijs and Jegou, Herve},
booktitle = {Advances in Neural Information Processing Systems (NeurIPS)},
pages = {8252--8262},
year = {2019},
}



@InProceedings{ECCV_18,
author="Mahajan, Dhruv
and Girshick, Ross
and Ramanathan, Vignesh
and He, Kaiming
and Paluri, Manohar
and Li, Yixuan
and Bharambe, Ashwin
and van der Maaten, Laurens",
title={{Exploring the Limits of Weakly Supervised Pretraining}},
booktitle={European Conference on Computer Vision (ECCV)},
year="2018",
pages="185--201",
}






@inproceedings{inception,
  author={Szegedy, Christian and Vanhoucke, Vincent and Ioffe, Sergey and Shlens, Jon and Wojna, Zbigniew},
  booktitle={2016 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={{Rethinking the Inception Architecture for Computer Vision}}, 
  year={2016},
  pages={2818-2826},
}







@INPROCEEDINGS{promise,
author={P. {Srivastava} and et al}, booktitle={2018 ACM/IEEE 45th Annual International Symposium on Computer Architecture (ISCA)}, 
title={{PROMISE: An End-to-End Design of a Programmable Mixed-Signal Accelerator for Machine-Learning Algorithms}}, 
year={2018}, 
pages={43-56},}




@INPROCEEDINGS{compute_caches, 
author={Aga, Shaizeen and Jeloka, Supreet and Subramaniyan, Arun and Narayanasamy, Satish and Blaauw, David and Das, Reetuparna}, 
booktitle={2017 IEEE International Symposium on High Performance Computer Architecture (HPCA)}, 
title={{Compute Caches}},
year={2017},
pages={481-492},}



@INPROCEEDINGS{ambit, 
author={V. {Seshadri} and et al}, 
booktitle={2017 50th Annual IEEE/ACM International Symposium on Microarchitecture (MICRO)},
title={{Ambit: In-Memory Accelerator for Bulk Bitwise Operations Using Commodity DRAM Technology}},
year={2017}, 
pages={273-287},}


@INPROCEEDINGS{neural_cache, 
author={C. {Eckert} and X. {Wang} and J. {Wang} and A. {Subramaniyan} and R. {Iyer} and D. {Sylvester} and D. {Blaaauw} and R. {Das}}, booktitle={2018 ACM/IEEE 45th Annual International Symposium on Computer Architecture (ISCA)}, 
title={{Neural Cache: Bit-Serial In-Cache Acceleration of Deep Neural Networks}},
year={2018},
pages={383-396},}


@inproceedings{dracc,
author = {Deng, Quan and Jiang, Lei and Zhang, Youtao and Zhang, Minxuan and Yang, Jun},
title = {{DrAcc: A DRAM Based Accelerator for Accurate CNN Inference}},
year = {2018},
pages={1--6},
booktitle = {Proceedings of the 55th Annual Design Automation Conference (DAC)},
}


@inproceedings{dram1,
author = {Gao, Fei and Tziantzioulis, Georgios and Wentzlaff, David},
title = {{ComputeDRAM: In-Memory Compute Using Off-the-Shelf DRAMs}},
year = {2019},
booktitle = {Proceedings of the 52nd Annual IEEE/ACM International Symposium on Microarchitecture (MICRO)},
pages = {100--113},
}




@INPROCEEDINGS{drisa, 
author={S. {Li} and D. {Niu} and K. T. {Malladi} and H. {Zheng} and B. {Brennan} and Y. {Xie}}, 
booktitle={2017 50th Annual IEEE/ACM International Symposium on Microarchitecture (MICRO)}, 
title={{DRISA: A DRAM-based Reconfigurable In-Situ Accelerator}}, year={2017},
pages={288-301},}




@article{lstm,
author = {Hochreiter, Sepp and Schmidhuber, Jürgen},
title = {{Long Short-Term Memory}},
journal = {Neural Computation},
volume = {9},
number = {8},
pages = {1735-1780},
year = {1997},
}

@inproceedings{gru,
title = {{Empirical Evaluation of Gated Recurrent Neural Networks on Sequence Modeling}},
author = {Junyoung Chung and et al},
year = "2014",
pages = {1--8},
booktitle = "Neural Information Processing Systems (NeurIPS) Workshop",
}



@INPROCEEDINGS{rram_pre, 
author={T. F. {Wu} and et al}, 
booktitle={2019 IEEE International Solid- State Circuits Conference (ISSCC)}, 
title={{A 43pJ/Cycle Non-Volatile Microcontroller with 4.7$\mu$s Shutdown/Wake-up Integrating 2.3-bit/Cell Resistive RAM and Resilience Techniques}},
year={2019}, 
pages={226-228},}


















@inproceedings{floatpim,
 author = {Imani, Mohsen and et al},
 title = {{FloatPIM}: {In-memory Acceleration of Deep Neural Network Training with High Precision}},
 booktitle = {2019 ACM/IEEE 46th Annual International Symposium on Computer Architecture (ISCA)},
 year = {2019},
 pages = {802--815},
 numpages = {14},
} 




@inproceedings{sparse_ReRAM,
 author = {Yang, Tzu-Hsien and et al},
 title = {{Sparse ReRAM Engine: Joint Exploration of Activation and Weight Sparsity in Compressed Neural Networks}},
 booktitle = {2019 ACM/IEEE 46th Annual International Symposium on Computer Architecture (ISCA)},
 year = {2019},
 pages = {236--249},
 numpages = {14},
}


@inproceedings{mei,
  title={Merging the interface: Power, area and accuracy co-optimization for rram crossbar-based mixed-signal computing system},
  author={Li, Boxun and et al},
  booktitle={Proceedings of the 52th Annual Design Automation Conference (DAC)},
  year={2015},
}

@inproceedings{enabling_sci,
  title={Enabling scientific computing on memristive accelerators},
  author={Feinberg, Ben and Vengalam, Uday Kumar Reddy and Whitehair, Nathan and Wang, Shibo and Ipek, Engin},
  booktitle={2018 ACM/IEEE 45th Annual International Symposium on Computer Architecture (ISCA)},
  pages={367--382},
  year={2018},
}

@article{u_approx,
  title={{Approximation Capabilities of Multilayer Feedforward Networks}},
  author={Hornik, Kurt},
  journal={Neural networks},
  volume={4},
  number={2},
  pages={251--257},
  year={1991},
}



@article{rram_approxi,
  title={{RRAM-Based Analog Approximate Computing}},
  author={Li, Boxun and Gu, Peng and Shan, Yi and Wang, Yu and Chen, Yiran and Yang, Huazhong},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems (TCAD)},
  volume={34},
  number={12},
  pages={1905--1917},
  year={2015},
}


@inproceedings{li2015variation,
  title={{Variation-Aware, Reliability-Emphasized Design And Optimization of RRAM using SPICE Model}},
  author={Li, Haitong and Jiang, Zizhen and Huang, Peng and Wu, Yi and Chen, H-Y and Gao, Bin and Liu, XY and Kang, JF and Wong, H-SP},
  booktitle={2015 Design, Automation Test in Europe Conference Exhibition (DATE)},
  pages={1425--1430},
  year={2015},
}








@Techreport{cifar,
 author = {Krizhevsky, Alex and Hinton, Geoffrey},
 address = {Toronto, Ontario},
 institution = {University of Toronto},
 publisher = {Technical report, University of Toronto},
 title = {{Learning Multiple Layers of Features from Tiny Images}},
 year = {2009},
}

@article{adc,
  title={{A 3.1 mW 8b 1.2 GS/s Single-Channel Asynchronous SAR ADC with Alternate Comparators for Enhanced Speed in 32 nm Digital SOI CMOS}},
  author={Kull, Lukas and Toifl, Thomas and Schmatz, Martin and Francese, Pier Andrea and Menolfi, Christian and Braendli, Matthias and Kossel, Marcel and Morf, Thomas and Andersen, Toke Meyer and Leblebici, Yusuf},
  journal={IEEE Journal of Solid-State Circuits (JSSC)},
  volume={48},
  number={12},
  pages={3049--3058},
  year={2013},
  publisher={IEEE}
}














@inproceedings{ji2018recom,
  title={{ReCom: An Efficient Resistive Accelerator for Compressed Deep Neural Networks}},
  author={Ji, Houxiang and et al},
  booktitle={2018 Design, Automation Test in Europe Conference Exhibition (DATE)},
  pages={237--240},
  year={2018},
}

@inproceedings{qiu2018peripheral,
  title={{A Peripheral Circuit Reuse Structure Integrated with a Retimed Data Flow for Low Power RRAM Crossbar-based CNN}},
  author={Qiu, Keni and et al},
  booktitle={2018 Design, Automation Test in Europe Conference Exhibition (DATE)},
  pages={1057--1062},
  year={2018},
}

@inproceedings{lin2019learning,
  title={{Learning the Sparsity for ReRAM: Mapping And Pruning Sparse Neural Network for ReRAM Based Accelerator}},
  author={Lin, Jilan and et al},
  booktitle={Asia and South Pacific Design Automation Conference (ASPDAC)},
  pages={639--644},
  year={2019},
}

@inproceedings{prime,
  title={{PRIME: A Novel Processing-In-Memory Architecture for Neural Network Computation in ReRAM-based Main Memory}},
  author={Chi, Ping and et al},
  booktitle={2016 ACM/IEEE 43rd Annual International Symposium on Computer Architecture (ISCA)},
  pages={27--39},
  year={2016},
}

@inproceedings{long2019design,
  title={{Design of Reliable DNN Accelerator with Un-reliable ReRAM}},
  author={Long, Yun and et al},
  booktitle={2019 Design, Automation Test in Europe Conference Exhibition (DATE)},
  pages={1769--1774},
  year={2019},
  organization={IEEE}
}

@inproceedings{pipelayer,
  title={{Pipelayer: A Pipelined Reram-based Accelerator for Deep Learning}},
  author={Song, Linghao and et al},
  booktitle={2017 IEEE International Symposium on High Performance Computer Architecture (HPCA)},
  pages={541--552},
  year={2017},
}

@inproceedings{hu2016dot,
  title={{Dot-Product Engine for Neuromorphic Computing: Programming 1T1M Crossbar to Accelerate Matrix-Vector Multiplication}},
  author={Hu, Miao and et al},
  booktitle={Proceedings of the 53rd Annual Design Automation Conference (DAC)},
  pages={1--6},
  year={2016},
}



@article{lecun1998gradient,
  title={{Gradient-Based Learning Applied to Document Recognition}},
  author={LeCun, Yann and et al},
  journal={Proceedings of the IEEE},
  volume={86},
  number={11},
  pages={2278--2324},
  year={1998},
}





@article{murmann2019adc,
  title={ADC performance survey 1997-2019},
  author={Murmann, Boris and others},
  journal={[Online] http://www.stanford.edu/murmann/adcsurvey.html},
  year={2019}
}

@article{saberi2011analysis,
  title={{Analysis of Power Consumption and Linearity in Capacitive Digital-to-Analog Converters Used in Successive Approximation ADCs}},
  author={Saberi, Mehdi and et al},
  journal={IEEE Transactions on Circuits and Systems I: Regular Papers (TCAS-I)},
  volume={58},
  number={8},
  pages={1736--1748},
  year={2011},
}






@ARTICLE{cao2019neuadc,
  author={W. {Cao} and X. {He} and A. {Chakrabarti} and X. {Zhang}},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems (TCAD)}, 
  title={{NeuADC: Neural Network-Inspired Synthesizable Analog-to-Digital Conversion}}, 
  year={2020},
  volume={39},
  number={9},
  pages={1841-1854},
}



@INPROCEEDINGS{cao2019neuadc_C,
  author={Cao, Weidong and He, Xin and Chakrabarti, Ayan and Zhang, Xuan},
  booktitle={2019 Design, Automation Test in Europe Conference Exhibition (DATE)}, 
  title={{NeuADC: Neural Network-Inspired RRAM-Based Synthesizable Analog-to-Digital Conversion with Reconfigurable Quantization Support}}, 
  year={2019},
  pages={1477-1482},
  }
  
  

@ARTICLE{adc_scal,
author={M. {Saberi} and R. {Lotfi} and K. {Mafinezhad} and W. A. {Serdijn}},
journal={IEEE Transactions on Circuits and Systems I: Regular Papers (TCAS-I)},
title={{Analysis of Power Consumption and Linearity in Capacitive Digital-to-Analog Converters Used in Successive Approximation ADCs}},
year={2011},
volume={58},
number={8},
pages={1736-1748},
month={Aug},}





@inproceedings{haq,
  author={Wang, Kuan and Liu, Zhijian and Lin, Yujun and Lin, Ji and Han, Song},
  booktitle={2019 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={{HAQ: Hardware-Aware Automated Quantization With Mixed Precision}}, 
  year={2019},
  pages={8604-8612},
}

@inproceedings{bit_fusion,
author = {Sharma, Hardik and et al},
title = {{Bit Fusion: Bit-Level Dynamically Composable Architecture for Accelerating Deep Neural Networks}},
year = {2018},
booktitle = {Proceedings of the 45th Annual International Symposium on Computer Architecture (ISCA)},
pages = {764--775},
}


@INPROCEEDINGS{quan_1,
  author={B. {Jacob} and S. {Kligys} and B. {Chen} and M. {Zhu} and M. {Tang} and A. {Howard} and H. {Adam} and D. {Kalenichenko}},
  booktitle={2018 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={{Quantization and Training of Neural Networks for Efficient Integer-Arithmetic-Only Inference}}, 
  year={2018},
  pages={2704-2713},}
  
  @inproceedings{quan_2,
  title={{Training and Inference with Integers in Deep Neural Networks}},
  author={Shuang Wu and Guoqi Li and Feng Chen and Luping Shi},
  booktitle={International Conference on Learning Representations (ICLR)},
  pages={1--10},
  year={2018},
}

@article{adam,
  title={{Adam: A Method for Stochastic Optimization}},
  author={Diederik P. Kingma and Jimmy Ba},
  journal={CoRR},
  year={2015},
  volume={abs/1412.6980}
}

@inproceedings{tf,
author = {Mart{\'\i}n Abadi and et al},
title = {{TensorFlow: A System for Large-Scale Machine Learning}},
booktitle = {12th {USENIX} Symposium on Operating Systems Design and Implementation ({OSDI} 16)},
year = {2016},
pages = {265--283},
}


@ARTICLE{rram_vari,
  author={F. {Bedeschi} and et al},
  journal={IEEE Journal of Solid-State Circuits (JSSC)}, 
  title={{A Bipolar-Selected Phase Change Memory Featuring Multi-Level Cell Storage}}, 
  year={2009},
  volume={44},
  number={1},
  pages={217-227},}
  
@article{dac,
  title={Analysis of Power Consumption and Linearity in Capacitive Digital-to-Analog Converters Used in Successive Approximation ADCs},
  author={Saberi, Mehdi and Lotfi, Reza and Mafinezhad, Khalil and Serdijn, Wouter A},
  journal={IEEE Transactions on Circuits and Systems I: Regular Papers (TCAS-I)},
  volume={58},
  number={8},
  pages={1736--1748},
  year={2011},
  publisher={IEEE}
}

@article{7bitReRAM,
  title={High precision tuning of state for memristive devices by adaptable variation-tolerant algorithm},
  author={Alibart, Fabien and Gao, Ligang and Hoskins, Brian D and Strukov, Dmitri B},
  journal={Nanotechnology},
  volume={23},
  number={7},
  pages={075201},
  year={2012},
}

@INPROCEEDINGS{pipelineadc,
  author={W. {Cao} and L. {Ke} and A. {Chakrabarti} and X. {Zhang}},
  booktitle={2019 IEEE/ACM International Conference on Computer-Aided Design (ICCAD)}, 
  title={{Neural Network-Inspired Analog-to-Digital Conversion to Achieve Super-Resolution with Low-Precision RRAM Devices}}, 
  year={2019},
  pages={1-7},
  }


@article{pipelineadc_J,
 author={Cao, Weidong and Ke, Liu and Chakrabarti, Ayan and Zhang, Xuan},
 journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems (TCAD)}, 
 title={{Evaluating Neural Network-Inspired Analog-to-Digital Conversion With Low-Precision RRAM}}, 
 year={2021},
 volume={40},
 number={5},
 pages={808-821},
 }
  
  
  
  

@article{sh,
  title={{A 10-nW 12-bit Accurate Analog Storage Cell with 10-aA Leakage}},
  author={O'Halloran, Micah and Sarpeshkar, Rahul},
  journal={IEEE Journal of Solid-State Circuits (JSSC)},
  volume={39},
  number={11},
  pages={1985--1996},
  year={2004},
  publisher={IEEE}
}


@ARTICLE{era-lstm,
  author={J. {Han} and H. {Liu} and M. {Wang} and Z. {Li} and Y. {Zhang}},
  journal={IEEE Transactions on Parallel and Distributed Systems (TPDS)}, 
  title={{ERA-LSTM: An Efficient ReRAM-Based Architecture for Long Short-Term Memory}}, 
  year={2020},
  volume={31},
  number={6},
  pages={1328-1342},}



% \end{thebibliography}



%%%%%% reference for the revision

@inproceedings{CNNWire,
author = {Lin, Jilan and Li, Shuangchen and Hu, Xing and Deng, Lei and Xie, Yuan},
title = {{CNNWire: Boosting Convolutional Neural Network with Winograd on ReRAM Based Accelerators}},
year = {2019},
booktitle = {Proceedings of the 2019 on Great Lakes Symposium on VLSI (GLVLSI)},
pages = {283–286},
numpages = {4},
}


==> discussion_envision.tex <==
\section{Discussion And Envision}
\label{sec:discuss}
Discussions and related works and envision.
